Transverse Single-Spin Asymmetries of Midrapidity Direct Photons, Neutral Pions, and Eta Mesons in 200 GeV Polarized Proton-Proton Collisions at PHENIX

Experimental observations of strikingly large transverse single-spin asymmetries (TSSAs) opened a window into quark and gluon dynamics present in hadronic collisions, revealing large spin-momentum correlations within nucleons and in the process of forming hadrons. Though originally measured in lower energy fixed target experiments, they have been found to persist in collisions with momentum transfer well into the perturbative regime of quantum chromodynamics (QCD) and yet their origin remains poorly understood. TSSA measurements have allowed for the development of both transverse momentum dependent and collinear twist-3 descriptions of nonperturbative spin-momentum correlations for both initial- and final-state effects. Results are presented for the TSSAs of direct photons, neutral pions, and eta mesons in the pseudorapidity range $|\eta|<0.35$ from $p^\uparrow+p$ collisions with $\sqrt{s} = 200$ GeV at PHENIX. As hadrons, $\pi^0$ and $\eta$ mesons are sensitive to both initial- and final-state effects. At midrapidity, $\pi^0$ and $\eta$ measurements are sensitive to the dynamics of gluons along with a mix of quark flavors. These results are a factor of three increase in statistical precision and extend to higher transverse momentum when compared with previous PHENIX measurements in this kinematic region. Because direct photon production does not include hadronization, the direct photon TSSA is only sensitive to spin-momentum correlations in the proton. The kinematics of this result in particular make the direct photon TSSA a clean probe of gluon dynamics in the transversely polarized proton. All three of these asymmetries will help constrain the twist-3 trigluon collinear correlation function as well as the gluon Sivers function, improving our knowledge of spin-dependent gluon dynamics in QCD.

==> abbr.tex <==
\acro{AU}{Astronomical Unit}
\acro{FIP}{first ionization potential}
\acro{MHD}{magnetohydrodynamic}
